A Comparison of Well-Quasi Orders on Trees

Well-quasi orders such as homeomorphic embedding are commonly used to ensure termination of program analysis and program transformation, in particular supercompilation. We compare eight well-quasi orders on how discriminative they are and their computational complexity. The studied well-quasi orders comprise two very simple examples, two examples from literature on supercompilation and four new proposed by the author. We also discuss combining several well-quasi orders to get well-quasi orders of higher discriminative power. This adds 19 more well-quasi orders to the list.

==> eptcsdata.tex <==
\providecommand{\firstpage}{30}
\providecommand{\publicationstatus}{A. Banerjee, O. Danvy, K.-G. Doh, J. Hatcliff (Eds):\\
David A. Schmidt's 60th Birthday Festschrift\\
EPTCS 129, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.129.3}{10.4204/EPTCS.129.3}}

